ImaGen: A General Framework for Generating Memory- and Power-Efficient Image Processing Accelerators

Image processing algorithms are prime targets for hardware acceleration as they are commonly used in resource- and power-limited applications. Today's image processing accelerator designs make rigid assumptions about the algorithm structures and/or on-chip memory resources. As a result, they either have narrow applicability or result in inefficient designs. This paper presents a compiler framework that automatically generates memory- and power-efficient image processing accelerators. We allow programmers to describe generic image processing algorithms (in a domain specific language) and specify on-chip memory structures available. Our framework then formulates a constrained optimization problem that minimizes on-chip memory usage while maintaining theoretical maximum throughput. The key challenge we address is to analytically express the throughput bottleneck, on-chip memory contention, to enable a lightweight compilation. FPGA prototyping and ASIC synthesis show that, compared to existing approaches, accelerators generated by our framework reduce the on-chip memory usage and/or power consumption by double digits.

==> sec_impl.tex <==
\section{Implementation Details}
\label{sec:impl}

We implement our compiler in Python with about 1,500 lines of code.
%We use Python so that we can quickly prototype and iterate over different ideas.
We use Google's optimization library ``or-tools''~\cite{ortools} for solving the ILP problem.

%Our code generator takes the schedule generated by the optimizer and produces System Verilog code.
We choose System Verilog as the code generation target because it has abstractions such as the \texttt{logic} keyword and diverse built-in math functions that make it easier to implement stencil operations.
The generated code has compute units to implement the stencil computations and memory blocks that implement line buffers as well as control logic to sequence the hardware.

For the compute units in each stage, our code maps computations in each stage to behavioral Verilog. The mapping is straightforward, since computations in each stencil operation involve only simple arithmetics.
%Structural Verilog, in theory, would provide more control over the hardware, but stencil computations are simple arithmetic operations for which structural Verilog is not necessary unless one has to design highly optimized processing units.
We do \textit{not} claim novelty at this step: one could plug RTL generated by other tools, e.g., an HLS, into our compiler at this step.
We replicate the processing element three times in each stage, one for processing a color channel.

One special care the code generator takes is that virtual stages that belong to the same physical stage read from a different, but offline-determined offset. For instance in \Fig{fig:lc}, $K2_2$ will always read from an offset of $W$ (image width) from \textsf{b1}, where $K2_1$ and $K1$ have an offset of 0.

%We use a 16-bit fixed-point data representation for intermediate data between stages. This might initially seem unnecessary, since each color in the input pixels is represented by 8 bits as in most of the color encodings.

%This is necessary, because intermediate computations might generate the fractional data; using a 8-bit representation would lose accuracy. %There are optimizations possible to use fewer bits\cite{??}, but the idea in this paper works independently of such optimizations.
%\fixme{could consider leaving this out.}
